Emergence of Shape Bias in Convolutional Neural Networks through Activation Sparsity

Current deep-learning models for object recognition are known to be heavily biased toward texture. In contrast, human visual systems are known to be biased toward shape and structure. What could be the design principles in human visual systems that led to this difference? How could we introduce more shape bias into the deep learning models? In this paper, we report that sparse coding, a ubiquitous principle in the brain, can in itself introduce shape bias into the network. We found that enforcing the sparse coding constraint using a non-differential Top-K operation can lead to the emergence of structural encoding in neurons in convolutional neural networks, resulting in a smooth decomposition of objects into parts and subparts and endowing the networks with shape bias. We demonstrated this emergence of shape bias and its functional benefits for different network structures with various datasets. For object recognition convolutional neural networks, the shape bias leads to greater robustness against style and pattern change distraction. For the image synthesis generative adversary networks, the emerged shape bias leads to more coherent and decomposable structures in the synthesized images. Ablation studies suggest that sparse codes tend to encode structures, whereas the more distributed codes tend to favor texture. Our code is host at the github repository: \url{https://github.com/Crazy-Jack/nips2023_shape_vs_texture}

==> fig_tex/shape_bias_benchmark.tex <==


\begin{figure}[ht!]
\centering
\includegraphics[width=0.8\textwidth]{figs/shapeBias_all.jpg}
\caption{TODO}
\label{fig:shape-bias-compare}
\end{figure}




==> fig_tex/supp_direct_vis.tex <==
\begin{figure}[ht!]
    \centering
    \includegraphics[width=\textwidth]{figs/FinalTopk_Sup1.pdf}
    \caption{Visualizing Top-K and non Top-K neurons through optimizing input images to match their activation. }
    \label{fig:my_label}
\end{figure}

==> sections/conclusion.tex <==
\section{Conclusion}

==> sections/proof.tex <==
\section{Proof}

To find the subgradient of the top-k operation, let's first define the operation and its input. Let $x \in R^n$ be an input vector, and let $T_k: R^n\rightarrow R^k$ be the top-k operation. The top-k operation $T_k(x)$ returns a vector $y \in R^k$ with the k highest values of x in descending order.

We will find the subgradient of the top-k operation with respect to the input x.

Since the top-k operation is piecewise linear, it is subdifferentiable. However, the subgradient may not be unique at the boundaries between linear regions. Therefore, we consider the subdifferential, which is a set of all possible subgradients at a given point.

% The subdifferential ∂T_k(x) can be defined element-wise. For each element x_i in the input vector x:

% 1. If x_i is among the top-k elements, the subgradient of T_k(x) with respect to x_i is 1. This is because increasing x_i by a small amount will result in an increase in the top-k elements.

% 2. If x_i is not among the top-k elements, the subgradient of T_k(x) with respect to x_i lies in the interval [0, 1]. This is because increasing x_i by a small amount may or may not affect the top-k elements, depending on the relative position of x_i compared to the top-k elements. In this case, the subdifferential ∂T_k(x) with respect to x_i is the entire interval [0, 1].

% So, the subdifferential of the top-k operation is a set of vectors g ∈ ℝ^n, where each element g_i ∈ [0, 1] if x_i is not in the top-k elements and g_i = 1 if x_i is in the top-k elements.


% for the reference of subgradient:
% https://web.stanford.edu/class/ee364b/lectures/subgradients_notes.pdf



Sparsifying Networks via Subdifferential Inclusion

Even if the Topk is not differentiable, with convolution, will it become smaller in variance?

\subsection{Optimizing for the boundary}

In this section, we show that the topk operator is optimizing for the boundary. 

CNN represents the shape by 




\subsection{Line drawing}

\paragraph{Strip Photograph to Line drawing doesn't impact representation too much}


Walther, Dirk B., et al. "Simple line drawings suffice for functional MRI decoding of natural scene categories." Proceedings of the National Academy of Sciences 108.23 (2011): 9661-9666. 




\subsection{Results for now}
First, we have the results of good performance of the 



==> tbl/texform_tbl.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% TexForm Results
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table}[h!]
% \fontsize{10}{12}\selectfont 
\large
\centering
\scalebox{0.60}{
\setlength{\arrayrulewidth}{.1em}
% \bigskip
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{c|cccccc}
\toprule
\multirow{2}[3]{*}{ Method} & \multicolumn{3}{c}{ImageNet Subset 1 (\textbf{IN-$S_1$})}  &\multicolumn{3}{c}{ImageNet Subset 2 (\textbf{IN-$S_2$})}\\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} 
 &Normal Acc. (\%)~$\uparrow$ & Shuffle-1 Acc. (\%)~$\downarrow$ & Shuffle-2 Acc. (\%)~$\downarrow$ & Normal Acc. (\%)~$\uparrow$ & Shuffle-1 Acc. (\%)~$\downarrow$ & Shuffle-2 Acc. (\%)~$\downarrow$ \\
\midrule
ResNet-18~\cite{he2016deep} & -49.0~$\pm$ -1.4    &-12.0~$\pm$ -1.9         & -43.5 / 47.5 / \cR & -12.5 / 13.8 / \cR   & -43.7 / 47.9 / \cR & -10.1/ 12.0 / \cR\\
ResNet-18~\cite{he2016deep} w. EC (ours)   & -\textbf{38.7}~$\pm$ 0.5 &-\textbf{5.9}~$\pm$ 0.7         & -\textbf{36.5 / 39.9 / 38.3} &-\textbf{7.2 / 7.6 / 5.9}    & -\textbf{39.6 / 41.3/ 39.7} &-\textbf{7.4 / 7.6 / 7.2}  \\
\bottomrule
\end{tabular}}
\vspace{2mm}
\caption{Few-shot Image Synthesis results measured in FID~\cite{heusel2018gans} and KID~\cite{binkowski2018demystifying} Note that KID * denotes KID scaled by a factor of $10^{3}$ to demonstrate the difference. }
% \vspace{-2mm}
\label{tb:main_performance_stylegan}
\end{table}






% \begin{table}[h!]
% \centering
% \scalebox{0.70}{
% \setlength{\arrayrulewidth}{.1em}
% % \bigskip
% \renewcommand{\arraystretch}{1.2}
% \begin{tabular}{c|cccccc}
% \toprule
% \multirow{2}[3]{*}{ Method} & \multicolumn{3}{c}{ImageNet Subset 1 (\textbf{IN-$S_1$})}  &\multicolumn{3}{c}{ImageNet Subset 2 (\textbf{IN-$S_2$})}\\
% \cmidrule(lr){2-4} \cmidrule(lr){5-7} 
%  &Normal Acc. (\%)~$\uparrow$ & Shuffle-1 Acc. (\%)~$\downarrow$ & Shuffle-2 Acc. (\%)~$\downarrow$ & Normal Acc. (\%)~$\uparrow$ & Shuffle-1 Acc. (\%)~$\downarrow$ & Shuffle-2 Acc. (\%)~$\downarrow$ \\
% \midrule
% ResNet-18~\cite{he2016deep} & -49.0~$\pm$ -1.4    &-12.0~$\pm$ -1.9         & -43.5 / 47.5 / \cR & -12.5 / 13.8 / \cR   & -43.7 / 47.9 / \cR & -10.1/ 12.0 / \cR\\
% ResNet-18~\cite{he2016deep} w. EC (ours)   & -\textbf{38.7}~$\pm$ 0.5 &-\textbf{5.9}~$\pm$ 0.7         & -\textbf{36.5 / 39.9 / 38.3} &-\textbf{7.2 / 7.6 / 5.9}    & -\textbf{39.6 / 41.3/ 39.7} &-\textbf{7.4 / 7.6 / 7.2}  \\
% \bottomrule
% \end{tabular}}
% \vspace{2mm}
% \caption{Few-shot Image Synthesis results measured in FID~\cite{heusel2018gans} and KID~\cite{binkowski2018demystifying} Note that KID * denotes KID scaled by a factor of $10^{3}$ to demonstrate the difference. }
% % \vspace{-2mm}
% \label{tb:main_performance_stylegan}
% \end{table}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% TexForm Results
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{figure}[ht!]
% \begin{floatrow}
% \capbtabbox{%
% \scalebox{0.8}{
% \setlength{\arrayrulewidth}{.1em}
% % \bigskip
% \renewcommand{\arraystretch}{1.2}
%     \begin{tabular}{cccc|ccc} \hline\hline
% Top-1 Acc. (\%)& IN-$S_1$ & Shuffled-IN-$S_1$ & Shuffled-IN-$S_1$ & IN-$S_2$ & Shuffled-IN-$S_2$ & Shuffled-IN-$S_1$\\ \hline\hline
%   ResNet-18~\cite{he2016deep} & \ph & \ph & \ph & \ph& \ph& \ph \\
%   ResNet-18 w. EC (Ours)  & \ph &  \ph & \ph & \ph& \ph & \ph\\ \hline
%   ResNet-18 w. ECM (Ours)  & \ph & \ph & \ph & \ph & \ph & \ph \\\hline\hline
%   \end{tabular}\label{tb:texform-1-results}
%     }
% }{%
%   \caption{10-category subsets from ImageNet~\cite{deng2009imagenet}.}%
% }


% \end{floatrow}
% \end{figure}
